Attenuation of Several Common Building Materials in Millimeter-Wave Frequency Bands: 28, 73 and 91 GHz

Future cellular systems will make use of millimeter wave (mmWave) frequency bands. Many users in these bands are located indoors, i.e., inside buildings, homes, and offices. Typical building material attenuations in these high frequency ranges are of interest for link budget calculations. In this paper, we report on a collaborative measurement campaign to find the attenuation of several typical building materials in three potential mmWave bands (28, 73, 91 GHz). Using directional antennas, we took multiple measurements at multiple locations using narrow-band and wide-band signals, and averaged out residual small-scale fading effects. Materials include clear glass, drywall (plasterboard), plywood, acoustic ceiling tile, and cinder blocks. Specific attenuations range from approximately 0.5 dB/cm for ceiling tile at 28 GHz to approximately 19 dB/cm for clear glass at 91 GHz.

==> Mahfuza_table_backup.tex <==
\begin{table*}[]
	\centering
	\caption{Average attenuation with standard variation at $28$, $73$ and $28$ GHz in three locations. $\sigma$ is the standard deviation of the penetration loss over
		all locations of a same material}
	\label{tab:resulst}
	\begin{tabular}{|c|c|c|c|c|c|c|}
		\hline
		Frequency                & Material          & Thickness, mm & Distance, cm & Attenuation, dB/cm & Mean attenuation, dB/cm          & Standard deviation dB, $\sigma$        \\ \hline
		
		\multirow{15}{*}{$91$ GHz} & \multirow{3}{*}{clear glass} & \multirow{3}{*}{$1.8$} &  $40$       &  $20.06$  & \multirow{3}{*}{$18.79$} & \multirow{3}{*}{$6.39$} \\ \cline{4-5}
		
		&                   &     &  $50$   &   $15.31$  &                   &                   \\ \cline{4-5}
		
		&                &   &     $60$     & $20.98$    &                   &                   \\ \cline{2-7} 
		
		& \multirow{3}{*}{plywood} &  \multirow{3}{*}{$11.2$}&   $40$      &   $9.65$  & \multirow{3}{*}{$11.76$} & \multirow{3}{*}{$4.2$} \\ \cline{4-5}
		&                   &    &  $50$    &  $12.64$   &                   &                   \\ \cline{4-5}
		
		&                &   &       $60$   &  $12.38$   &                   &                   \\ \cline{2-7} 
		
		& \multirow{3}{*}{drywall} &  \multirow{3}{*}{$13.1$} &  $40$       &   $1.78$  & \multirow{3}{*}{$1.97$} & \multirow{3}{*}{$1.26$} \\ \cline{4-5}
		&            &       &       $50$   &  $2.15$   &                   &                   \\ \cline{4-5}
		
		&                 &  &    $60$      &    $1.97$ &                   &                   \\ \cline{2-7}
		
		& \multirow{3}{*}{concrete} &  \multirow{3}{*}{$195$}& $40$       &  No signal detected    & \multirow{3}{*}{-} & \multirow{3}{*}{-} \\ \cline{4-5}
		&               &    &       $50$   &  No signal detected    &                   &                   \\ \cline{4-5}
		
		&          &         &    $60$      &    No signal detected  &                   &                   \\ \cline{2-7}
		
		& \multirow{3}{*}{acoustic ceiling} &  \multirow{3}{*}{$11.3$}&  $40$      &    $2.01$ & \multirow{3}{*}{} & \multirow{3}{*}{} \\ \cline{4-5}
		&         &          &      $50$    &     &                   &                   \\ \cline{4-5}
		
		&        &           &        $60$  &     &                   &                   \\ \hline
		
		
		
		
		 \multirow{15}{*}{$73$ GHz} & \multirow{3}{*}{clear glass} & \multirow{3}{*}{$1.8$}&    $40$       &  $15.34$  & \multirow{3}{*}{$14.37$} & \multirow{3}{*}{$5.76$} \\ \cline{4-5}
		
		&        &           &       $50$   &   $15.87$  &                   &                   \\ \cline{4-5}
		
		&           &        &     $60$     & $11.9$    &                   &                   \\ \cline{2-7}
		 
		& \multirow{3}{*}{plywood} &   \multirow{3}{*}{$11.2$}&  $40$      &   $6.79$  & \multirow{3}{*}{$7.14$} & \multirow{3}{*}{$0.81$} \\ \cline{4-5}
		&       &            &      $50$    &  $6.67$   &                   &                   \\ \cline{4-5}
		
		&         &          &       $60$   &  $7.9$   &                   &                   \\ \cline{2-7}
		
		
		& \multirow{3}{*}{drywall} &  \multirow{3}{*}{$13.1$}&  $40$       &   $1.76$  & \multirow{3}{*}{$1.45$} & \multirow{3}{*}{$0.73$} \\ \cline{4-5}
		&          &         &       $50$   &  $0.76$   &                   &                   \\ \cline{4-5}
		&          &         &    $60$      &    $1.84$ &                   &                   \\ \cline{2-7}
		
		& \multirow{3}{*}{concrete} &  \multirow{3}{*}{$195$}&  $40$       &  No signal detected   & \multirow{3}{*}{-} & \multirow{3}{*}{-} \\ \cline{4-5}
		&        &           &       $50$   &  No signal detected    &                   &                   \\ \cline{4-5}
		&         &          &    $60$      &    No signal detected  &                   &                   \\ \cline{2-7}
		
		
		& \multirow{3}{*}{acoustic ceiling} &   \multirow{3}{*}{$11.3$}&  $40$      &    $0.85$ & \multirow{3}{*}{$0.93$} & \multirow{3}{*}{$.52$} \\ \cline{4-5}
		&           &        &      $50$    &  $1.09$   &                   &                   \\ \cline{4-5}
		
		&        &           &        $60$  &  $0.86$   &                   &                   \\ \hline
		
		
		
		
		\multirow{15}{*}{$28$ GHz} &  \multirow{3}{*}{clear glass} &  \multirow{3}{*}{$1.8$} &  $40$       &  $4.26$  & \multirow{3}{*}{$4.38$} & \multirow{3}{*}{$0.18$} \\ \cline{4-5}
		
		&           &        &       $50$   &   $4.44$  &                   &                   \\ \cline{4-5}
		
		&          &         &     $60$     & $4.44$    &                   &                   \\ \cline{2-7}
		
		& \multirow{3}{*}{plywood} &   \multirow{3}{*}{$11.2$}&  $40$      &   $4.73$  & \multirow{3}{*}{$5.09$} & \multirow{3}{*}{$1.28$} \\ \cline{4-5}
		&        &           &      $50$    &  $5.0$   &                   &                   \\ \cline{4-5}
		
		&          &         &       $60$   &  $5.57$   &                   &                   \\ \cline{2-7} 
		
		& \multirow{3}{*}{drywall} &   \multirow{3}{*}{$13.1$}&  $40$       &   $0.92$  & \multirow{3}{*}{$0.94$} & \multirow{3}{*}{$0.23$} \\ \cline{4-5}
		&         &          &       $50$   &  $0.69$   &                   &                   \\ \cline{4-5}
		&          &         &    $60$      &    $1.22$ &                   &                   \\ \cline{2-7}
		
		& \multirow{3}{*}{concrete} &  \multirow{3}{*}{$195$}&  $40$       &   $3.68$  & \multirow{3}{*}{$3.8$} & \multirow{3}{*}{$0.22$} \\ \cline{4-5}
		
		&        &           &       $50$   & $3.7$    &                   &                   \\ \cline{4-5}
		&        &           &    $60$      &    $4.10$ &                   &                   \\ \cline{2-7}
		
		& \multirow{3}{*}{acoustic ceiling} &  \multirow{3}{*}{$11.3$}&   $40$      &    $0.38$ & \multirow{3}{*}{$0.44$} & \multirow{3}{*}{$0.06$} \\ \cline{4-5}
		&         &          &      $50$    &  $0.47$   &                   &                   \\ \cline{4-5}
		
		&      &             &        $60$  &  $0.47$   &                   &                   \\ \hline
		
		
	\end{tabular}
\end{table*}



%%%%%%%%
